Quantum Annealing based Feature Selection in Machine Learning

Feature selection is crucial for enhancing the accuracy and efficiency of machine learning (ML) models. This work investigates the utility of quantum annealing for the feature selection process in an ML-pipeline, used for maximizing the mutual information (MI) or conditional mutual information (CMI) of the underlying feature space. Calculating the optimal set of features that maximize the MI or CMI is computationally intractable for large datasets on classical computers, even with approximative methods. This study employs a Mutual Information Quadratic Unconstrained Binary Optimization (MIQUBO) formulation, enabling its solution on a quantum annealer. We demonstrate the capability of this approach to identify the best feature combinations that maximize the MI or CMI. To showcase its real-world applicability, we solve the MIQUBO problem to forecast the prices of used excavators. Our results demonstrate that for datasets with a small MI concentration the MIQUBO approach can provide a significant improvement over MI-only based approaches, dependent on the dimension of the selected feature space.

==> Bharadwaj_abstract.tex <==
\section{\uppercase{Introduction}}
\label{sec:introduction}


The paper presents a novel approach to feature selection using mutual information and quantum computing resources, specifically D-Wave quantum annealers and hybrid solvers. The results reveal insights into the mutual information of features in the Caterpillar 308 dataset, highlighting the significance of certain features, such as construction year and working hours, in determining the price of used excavators. The study also demonstrates the effectiveness of the Mutual Information QUBO (MIQUBO) method in identifying the best feature combinations that maximize mutual information. The findings offer valuable implications for feature selection in machine learning and data analysis, showcasing the potential of quantum computing in addressing complex optimization tasks.

==> Computational_details.tex <==




